Work-in-Progress: A Simulation Framework for Domain-Specific System-on-Chips

Heterogeneous system-on-chips (SoCs) have become the standard embedded computing platforms due to their potential to deliver superior performance and energy efficiency compared to homogeneous architectures. They can be particularly suited to target a specific domain of applications. However, this potential is contingent upon optimizing the SoC for the target domain and utilizing its resources effectively at run-time. Cycle-accurate instruction set simulators are not suitable for this optimization, since meaningful temperature and power consumption evaluations require simulating seconds, if not minutes, of workloads. This paper presents a system-level domain-specific SoC simulation (DS3) framework to address this need. DS3 enables both design space exploration and dynamic resource management for power-performance optimization for domain applications with$~600\times$ speedup compared to commonly used gem5 simulator. We showcase DS3 using five applications from wireless communications and radar processing domain. DS3, as well as the reference applications, will be shared as open-source software to stimulate research in this area.

==> files/acknowledgement.tex <==
\section*{Acknowledgement} \label{sec:Acknowledgement}
This material is based on research sponsored by Air Force Research Laboratory (AFRL) and Defense Advanced Research Projects Agency (DARPA) under agreemnet number FA8650-18-2-7860. The U.S. Government is authorized to reproduce and distribute reprints for Governmental purposes notwithstanding any copyright notation thereon. 
The views and conclusion contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either expressed or implied, of Air Force Research Laboratory (AFRL) and Defence Advanced Research Projects Agency (DARPA) or the U.S. Government.

==> files/backup.tex <==
Heterogeneous system-on-chip (SoC) architectures efficiently combine the advantages of both classes of architectures. 
Integration of general-purpose processors, special-purpose cores and custom accelerators provide far superior performance at reduced energy footprint compared to their homogeneous counterparts. 
Domain-specific SoCs, a class of heterogeneous architectures, exploit characteristics and behavior of applications in a particular domain to make design choices that optimize peak performance per watt (PPW). 
Hence, heterogeneous platforms are very suitable for PPW efficient computations in emerging application domains such as machine learning, artificial intelligence, natural language processing and autonomous driving.


Heterogeneous architectures offer improved energy efficient computations but also pose significant challenges in terms of design choices and architecture tuning. 
Resource and power-thermal management of the platform are some of the more concerning challenges.
%This leads to increase in development cost of the SoC.
The challenges are exacerbated by heterogeneity and large numbers of processing elements (PEs) in typical architectures. 
Aggressive optimization is often limited due to complexities introduced by stringent power and energy constraints. 
The time consumed in architecture exploration is very high and not affordable with today's quick time-to-market requirements. Hence, there is a need to circumvent the challenges and improve the design space exploration process.




~\cite{hennessy2019new}

Three steps
First, select the processors
Second, map/schedule them
Final step, and the focus of this paper, 


Heterogeneous system-on-chips (SoCs) span the gap between the flexibility of general-purpose processors and the energy-efficiency of specialized accelerators. Indeed, tailoring the architecture to characteristics of the target domain has been recognized as the most effective architectural approach to achieve higher efficiency~\cite{hennessy2019new}.
For example, mobile SoCs integrate low-power (little) and high-performance (big) cores with a variety of specialized processors, such as graphics processing units (GPUs), audio processors, and wireless modems~\cite{gupta2016generic}. 
Heterogeneous SoCs have dominated the mobile platform market by combining the ease of programming and superior energy-efficiency in mobile application scenarios~\cite{shin201328nm}.
However, no single SoC can satisfy the needs of unbounded applications domains due to area and cost constraints. 
Therefore, there is a strong need for approaches to formally identify application domains and design domain-specific system-on-chips (DSSoC). 

The design of DSSoCs entails five tightly coupled challenges, as summarized in Figure~\ref{fig:overview}. 
First, to encapsulate the intuition for a domain of applications and their computation requirements, the objective and quantitative definition of the target domain must be developed. 
For example, the most frequently used class of kernels, such as fast Fourier transforms (FFT), must be identified during this stage.
These classes represent the most promising candidates for generalized hardware acceleration. 
With this understanding, the designers can determine the type and number of processing elements (PE) that need to be employed in the DSSoC. 
The second challenge is to design hardware accelerators tailored to the major kernels identified in the target domain.
This step must optimize the balance between the effort of designing fixed function accelerators for this kernel 
and re-use of hardware resources among multiple kernels. 
The third challenge is to design the network-on-chip architecture that will interconnect all of the PEs 
to satisfy both on-chip and off-chip communication requirements between the PEs and external memory. 
Accelerator-rich architectures are notoriously known to be difficult to program. 
Hence, the DSSoC can be impractical unless the hardware resources can be used 
seamlessly to run the domain application. 
This capability is crucial to relieve the users from the details of the hardware design.
Therefore, the fourth challenge is to design a dynamic resource manager (DRM) 
that can optimally utilize the DSSoC at runtime.
The fifth challenge, a practical solution also requires a complete software stack that includes compiler support, 
programming tools and OS. 
Therefore, the fifth and final challenge is to design a companion software stack for DSSoCs. 

% I'll add an overview picture.

%is there a vector version of this? if not, it needs to be shortened to fit in the page - Rick
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/overview_picture.png}
    \caption{The overview of the five major steps of Domain-specific SoC Design. This paper focuses on the Ontological Inference problem highlighted in this figure.}
    \label{fig:overview}
\end{figure}


\begin{wrapfigure}{o}{0.45\linewidth}
\vspace{-8mm}
  \begin{center}
    \includegraphics[width=0.38\textwidth]{figures/HiLvlOntology.pdf}
  \end{center}
  \caption{Domain ontology is generated  by machine learning the relation between the inferred mathematical ontology and device ontology. It enables deriving the mapping, specification, and PE placements.}
  \label{fig:ontology}
  \vspace{-8mm}
\end{wrapfigure}  


Each of these challenges require significant research effort to make DSSoCs practical. 
Early work on application mapping to many-core architectures~\cite{hu2005energy} pioneered numerous solutions for both static and run-time mapping and scheduling approaches~\cite{sahu2013survey,hu2004energy,chou2008energy}. 
Similarly, a wide range of work addresses design of the network-on-chip architectures
and dynamic resource management under highly varying workloads~\cite{tatas2014designing,ogras2013modeling,xiao2017load,gupta2017dypo}. 
The goal of this paper is to present the ground-work for an ontological-inference framework that automatically analyzes target application-sets, learns their organization and structure, and optimizes selection of hardware resources.
Such a framework can be be used with existing techniques that target the other challenges. 
Specifically, we focus on the process of data-mining existing applications in order to build those ontologies.



==> files/capabilities.tex <==
% \section{User View: DS3 Capabilities} \label{sec:capabilities}

% This section presents the built-in scheduling and DTPM algorithms, and utilities provided to DS3 users.

% \subsection{Built-In Schedulers} \label{scheduler}



% DS3 provides a set of commonly used built-in scheduling algorithms, 
% which can be specified by the users in the main configuration file. 
% It also automatically generates  Gantt charts that depict the execution flow based on task to PE mapping decision made by the scheduler for a given job injection rate. 
% This allows the end-user to understand the dynamics of the scheduler under investigation, 
% as illustrated in this section. 
% We describe the built-in scheduling algorithms in DS3 using one of the most commonly used canonical task graphs~\cite{Topcu} shown in Figure~\ref{dag}. 
% Since this task graph is used commonly as a reference point across many list-scheduling studies, 
% it serves as a representative example before analyzing the results from real-world applications in Section~\ref{ssec:case_studies}.


% \noindent\textbf{Minimum Execution Time (MET) Scheduler: } 
% The MET scheduler assigns a ready task to a PE that achieves the minimum expected execution time following a first-in, first-out policy~\cite{heuristic_comparison}. 
% If there are multiple PEs that satisfy the minimum execution criterion, then the scheduler reads the current state information of all these PEs and assign the tasks to one of the idle PEs. 


% Figure~\ref{fig:schedule}(a) shows the schedule generated by the MET scheduler in DS3 for our running example (Figure~\ref{dag}). All tasks are assigned to their best-performing PEs as expected.

% \noindent\textbf{Earliest Task First (ETF) Scheduler:} 
% The ETF scheduler utilizes the information about the communication cost between tasks and the current status of all PEs while making the scheduling decision~\cite{workflow_schedule}. 
% Consider a set of PEs $P = \left\{p_0, p_1, ..., p_{q-1}\right\}$ and a task graph with tasks $N = \left\{n_0, n_1, ..., n_{k-1}\right\}$. For every task and PE pair we define the following quantities:
% \begin{itemize}[leftmargin=5mm]
%     \item { \textit{Estimated Execution Time}, $EET(n,p)$}, is the total amount of time that the resource $p$ takes to run the task $n$.

%     \item { \textit{Estimated Availability Time}, $EAT(n,p)$}, is defined as the time when the resource $p$ will finish executing all tasks in its queue before the task $n$.
    
%     \item { \textit{Data Availability Time}, $DAT(n,p)$}, is the earliest time at which all required data becomes available at resource $p$ to perform task $n$.

%     \item { \textit{Estimated Completion Time}, $ECT(n,p)$}, is the completion time of task $n$ executed on resource $p$. It is given by:
%     \begin{equation}
%     \ ECT(n,p) = EET(n,p) + max(EAT(n,p),DAT(n,p))
%     \end{equation}
% \end{itemize}

% The ETF scheduler finds the resource with the minimum $ECT$ value for each available task. Next, the task with the minimum $ECT$ value is determined and it is scheduled first. This routine is performed until all available tasks are assigned to a PE.

% Figure~\ref{fig:schedule}(b) shows the schedule, generated and plotted by the DS3, for the single instance of the task flow graph shown in Figure~\ref{dag} based on the ETF scheduler.
% Although the execution times are same for both MET and ETF based schedules, the mapping decisions are different as shown in Figure~\ref{fig:schedule}(a) and ~\ref{fig:schedule}(b). 
% This difference will become evident when we present the performance results for different applications 
% in Section~\ref{ssec:case_studies}.

% \noindent\textbf{Table-based Scheduler:} 
% DS3 also provides a scheduler which stores the scheduling decisions in a look-up table.  
% This allows users to utilize any offline schedule, such as an assignment generated by an integer linear programming (ILP) solver, with the help of a small look-up table. 
% For example, we used IBM ILOG CPLEX Optimization Studio~\cite{cplex} to generate the ILP solution for a single job instance of our running example. 
% The schedule from the ILP solution, depicted in Figure~\ref{fig:schedule}(c) 
% outperforms the other two schedulers for a single job instance as expected. 
% However, we note that the schedule stored in the table guarantees optimality only if there is a single job instance in the system. Therefore, its performance will degrade when multiple jobs overlap, as we demonstrate it 
% in Section~\ref{ssec:case_studies}.

% \subsection{Built-In DTPM Policies} \label{sec:dtpm}

% State-of-the-art SoCs support multiple voltage-frequency domains and dynamic voltage-frequency scaling (DVFS), which enables users to optimize various power-performance trade-offs.
% To support this capability, DS3 allows each PE to have a range of \textit{Operating Performance Points} (OPPs) that can be configured in the resource database. 
% The OPPs are voltage-frequency tuples that represent all supported frequencies of a given PE, 
% which can be exploited by DTPM algorithms to tune the system to the application at hand.
% In addition, DS3 integrates analytical power consumption and thermal models for the PEs stored in the resource database. 

% The power models capture both dynamic and static power consumption. 
% The dynamic power consumption ($P=CV^2Af$) varies according to the load capacitance (\textit{C}), supply voltage (\textit{V}), activity factor (\textit{A}), and operating frequency (\textit{f}). 
% Voltage and frequency are modeled through the OPPs, 
% while the load capacitance and activity factors are modeled using measurements on real devices and published data. 
% For example, we characterized Arm A57 and A53 power consumption on a Nexus 6P phone using our own setup. 
% We have integrated publicly available Arm A15 and A7 power consumption and temperature models available online~\cite{bhat2018algorithmic}, as well as published power consumption numbers for FFT ~\cite{chen2018variable} and Viterbi accelerators ~\cite{tobola2018low}.
% Finally, we use Cacti for cache and memory associated power models ~\cite{thoziyoor2008cacti}.
% The thermal models are obtained from measurements on Odroid-XU3~\cite{ODROID}. 
% %\todo{Dr. Marculescu: Below, there is no discussion on thermal models.}
% % 
% %  Dr. Marculescu: Below, there is no discussion on thermal models
% % 

% The integrated power, performance, and temperature models enable us to implement a wide range of DTPM policies using DS3. 
% %  We just gave refs at the previous paragraph.
% To provide a solid baseline to the user, we also provide built-in DVFS policies that are commonly implemented in commercial SoCs. 
% More specifically, users use the input configuration file to set the DTPM policy to \textit{Ondemand, Performance, Powersave} governors, or to a user-specified fixed value.

% \noindent \textbf{Ondemand Governor:} The Ondemand governor controls the OPP of each PE as a function of its utilization~\cite{pallipadi2006ondemand}. 
% The supported voltage-frequency pairs of a given PE are given by the following set: 
% \begin{equation} \label{Vf_pairs}
%     \mathcal{OPP} = \{(V_1, f_1), (V_2, f_2), \ldots, (V_n,f_n)\}
% \end{equation}
% where $n$ is the number of operating points supported by that PE. 
% Suppose that the PE currently operates at $(V_2, f_2)$.
% If the utilization of the PE is less than a user-defined threshold, then the Ondemand governor decreases the frequency and voltage such that the new OPP becomes $(V_1, f_1)$. 
% If the utilization is greater than another user-defined threshold, the OPP increases to $(V_3, f_3)$. 
% Otherwise, the OPP stays at the current value, i.e., $(V_2, f_2)$.

% \noindent \textbf{Performance Governor:} This policy sets the frequency of voltage of all PEs to their \textit{maximum values} to minimize execution time.
% % 
% %  Dr. Marculescu: This is basic staff. Not sure if we can't do better
% % 
% \noindent \textbf{Powersave Governor:} This policy sets the frequency and voltage of all PEs to their \textit{minimum values} to minimize power consumption.

% \noindent \textbf{User-Specified Values:} This policy enables users to set the OPP (i.e., frequency and voltage) of each PE individually to a constant value within the permitted range. It enables thorough power performance exploration by simply sweeping the supported values.

% Finally, developers can also define custom DTPM algorithms in the \textit{DTPM} class, similar to the scheduler. 

% \subsection{Built-in Utilities} \label{sec:validation}
% Developing new resource management algorithms is an arduous task involving many iterations. 
% Bearing this in mind, DS3 offers various tools to help and guide developers and users. 

% \noindent\textbf{Application logging} is an important tool in debugging application execution. 
% DS3 enables logging detailed messages at various levels. 
% The framework uses two-level classification of messages: (a) Type (information or debug) and (b) Source (configuration, scheduler or simulation).
% This utility of DS3 makes it convenient for users to understand the dynamics of simulation in the framework with ease.

% \noindent\textbf{Validation} is critical in development and simulation environments to ensure accuracy and reliability.
% In DS3, the sanity checks include (a) Comparison of the number of generated and completed jobs (refer to Figure~\ref{queues}) and (b) Ensure tasks execute only on compatible PEs.
% We ensure that simulation results are reliable by adding necessary assertions in the framework.
 
% \noindent\textbf{Regression Analysis} helps in the validation of newly implemented features and algorithms. 
% DS3 provides the utilities to perform regressions for developers to validate their changes in comparison to reference results and aids in the identification of faulty modifications.
% This capability helps in making DS3 scalable for simultaneous use by a large group of developers.

% % \nirmal{Its not clear to me that what regression utility has to do with the simultaneous usability by multiple users. Regression can be done by a single user.}
% % \samet{Yes regression can be done by a single user but if many people involves developing an algorithm for example, it will help them to have a golden version. this helps actually to developers instead of users so I changed users to developers. I hope now it make more sense.}


==> files/conclusion.tex <==
\section{Conclusion and Future Work}\label{sec:concandfuture}
\label{sec:CandF}

% The performance and energy efficiency potential of DSSoCs remains untapped unless we employ efficient run-time resource management techniques. 
% In this paper, we presented DS3, a Python-based open-source system-level framework for rapid design space exploration of domain specific SoCs. 
% We developed a scalable, modular, and flexible simulation framework to evaluate scheduling algorithms, dynamic power-thermal management techniques and architecture exploration. 
% We also presented benchmark applications, built-in scheduling algorithms and built-in DVFS policies which can be used as reference by users and developers.

% We will share DS3, built-in schedulers, DVFS governors and benchmark applications to the public to encourage research in the domain of DSSoCs.
% We identify the integration of learning-based schedulers and expanding the domain beyond wireless communications and radar systems as part of future scope of this work.



==> files/implementation.tex <==


% \section{\hspace{-2mm} Developer View: DS3 Implementation} \label{sec:implementation}

% \label{sec:Design}

% This section describes the implementations of the major components of 
% DS3 depicted in Figure~\ref{fig:DS3-framework} from a developer's perspective.

% \subsection{Resource Database} \label{sec:resource_database}

% DS3 can instantiate a wide range of SoC configurations with different types of general and special purpose PEs. 
% The list of PEs available to the user is stored in the resource database, 
% the first component of DS3, shown in Figure~\ref{fig:DS3-framework}. 
% Each PE in the database has the following \textit{static attributes}:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Type:} The type attribute defines the type of the PE, e.g., CPU, accelerator, etc. 
    
%     \item \textbf{Parallel processing capability:} This attribute is the number of threads that the PE can run in parallel. 
    
%     \item \textbf{DVFS policy:} This attribute is the DVFS policy for the PE, which controls frequency and voltage at run-time.
    
%     \item \textbf{Operating performance points (OPPs):} OPPs give the operating frequencies and the corresponding voltages for the PE.
    
%     \item \textbf{Execution time profile:} This attribute defines the execution time of an application on the PE, running at maximum frequency.
    
%     \item \textbf{Power consumption profile:} This attribute provides information about the power consumption of an application on the PE.
    
% \end{itemize}

% Each component also has a \textit{dynamic attribute} which states whether a PE is busy or idle.
% These attributes are used by the schedulers and DTPM governor to make their respective decisions, as described in Section~\ref{sec:capabilities}.
% For example, when a scheduler assigns a task to a specific type of PE, it can receive the state information of all PEs with the same type and schedule the task to an idle PE.

% Along with the list of available PEs, the shared memory is also listed as a PE in the resource database, with only the \textit{type attribute}.
% Finally, the database also contains the bandwidth information among all the PEs. This information is also utilized by the analytical latency model to estimate interconnect delay.

% % \todo{explain the state and how it is used at runtime.}

% % \todo{(a) and (c) below are \textbf{User Inputs} (e.g., (a) defines the SoC, (c) is for apps). 
% % They need to be explained in section 5. Simple examples would be also very useful}.

% \subsection{Job Generator}
% In DS3, we define a job as an instance of an application. 
% As an example, Figure ~\ref{fig:wifi_bd} presents a block diagram for a WiFi transmitter (WiFi-TX) job that is composed of multiple tasks. The dependency among the tasks is represented using a DAG. 
% Hence, the job generator produces the tasks, as shown in Figure~\ref{fig:wifi_bd}, for a transmitter job along with their dependencies. 
% The basic unit of data processed by this chain is a frame,
% which is 64 bits in this work. 
% Hence, each job implies a 64-bit frame streaming through the WiFi-TX chain. 
% If we assume that the jobs are separated on average by 10${\mu}s$, 
% this implies 6.4MB/s transmit rate.
% %  Nirmal: I am not sure how this description is related to the job generator. As we introduce WiFi later in the paper as a benchmark, we can just add a line here saying that "WiFi-TX is one of the benchmark available with DS3 and presented later in this work

% In general, the job generator produces the tasks and DAG for each active application following a user-specified traffic model.
% DS3 currently models the traffic by injecting jobs from an exponential distribution, but it provides flexibility to model other distributions as well. The framework is scalable in terms of job generation and is capable of spawning jobs from one or more applications in a predefined ratio.
% For example, suppose that both WiFi transmitter and WiFi receiver (WiFi-RX) applications are active. 
% DS3 can generate jobs for both applications following a user-specified WiFi-TX:WiFi-RX ratio and injection rate. 
% This capability enables exploring single application and multiple simultaneous application scenarios, as we demonstrate in Section~\ref{sec:case studies}. 

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=1\linewidth]{figures/WIFI_BD.png}
% 	\caption{Block diagram of WiFi application}
% 	\label{fig:wifi_bd}
% \end{figure}

% \subsection{Scheduling and DTPM Algorithms}

% DS3 enables a plug-and-play interface to choose between different scheduling and DTPM algorithms at run-time. 
% Hence, developers can implement their own algorithms and integrate them easily with DS3. 
% To achieve this, the developers need to define the new scheduling algorithm as a member function of the \textit{Scheduler class}. 
% Then, the new scheduler can be called easily from the \textit{run} method of the simulation core.

% Since there may be a wide range of custom algorithms with different complexities, DS3 requires a loosely defined interface. 
% The minimum set of inputs to these algorithms is a reference to the resource database  (Section~\ref{sec:resource_database}). 
% In this way, new algorithms can make informed decisions to utilize the available resources. 
% For example, a scheduler can access the set of idle PEs and 
% their power-performance profiles for running specific tasks. 
% In addition, the developer can provide other inputs, such as, 
% the set of tasks waiting to be scheduled and their dependencies. 

% The minimum required output for the scheduler is the assignment of the next available task to a PE. 
% If the PE is not idle at the time of the decision, DS3 places the task into the \textit{Executable Queue} as shown in Figure~\ref{queues}. 
% % \todo{Figure~\ref{queues} is not yet introduced. It is introduced in next section (4.4).}
% Otherwise, the execution starts in the following simulation cycle. 
% % ###########################################################
% % \todo{(Pls. make sure that the following sentence uses the same terminology as the related work.)}
% % ##########################################################
% DS3 also supports the List schedulers, such as HEFT~\cite{Topcu}, where schedule for all the tasks in a job is generated at the time of its submission (see~Figure\ref{queues}).


% Similar to schedulers, DS3 provides built-in DTPM policies and 
% facilitates design of new DTPM algorithms. 
% The DTPM policy is invoked periodically at every control epoch, 
% whose length is a user-controllable parameter. 
% To minimize the run-time and power consumption of DTPM decisions, 
% we use 10ms--100ms range following the common practice~\cite{bhat2018algorithmic}.
% The minimum set of inputs to the DTPM policy is the current power states of the PEs. 
% Advanced algorithms can also use PE utilization and more detailed performance metrics, such as number of memory accesses or retired instructions.
% %  Anderson: we do not have these metrics now.
% In addition, the DTPM policies have access to the resource management, including the power consumption and performance profiles therein. 
% The outputs of the DTPM algorithms are the power states of PEs in the next control epoch.
% These states are applied to the PEs until the DTPM policy is called again.

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{figures/Queues.png}
% 	\caption{Life-cycle of a task based on DS3 queues}
% 	\label{queues}
% \end{figure}


% \subsection{Simulation Kernel}
% %  Nirmal: It might be good to introduce simulation kernel before introducing scheduling and DTPM algorithms. As the terminology and figure from this section is used earlier. Further, the scheduler and DTPM are parts of simulation kernel.
% The core functionality of DS3 is implemented in the simulation kernel described in Figure~\ref{queues}. 
% The job generator thread produces batches of new tasks and the DAG that defines their dependencies for each active application.
% The first task in each new job, i.e., the head task, is directly written to the \textit{Ready Queue} 
% since it does not have any dependencies. 
% The tasks with dependencies are stored in the \textit{Outstanding Queue} where they wait for the completion of their predecessors.

% The scheduler thread is called whenever a new task is written to the \textit{Ready Queue}, as shown in Figure~\ref{queues} . 
% Simple schedulers, such as the minimum execution time scheduler, read only the contents of the \textit{Ready Queue}, 
% while complex schedulers can analyze the remaining DAG of running and waiting tasks to make next scheduling decision. 
% After the scheduler completes the task assignments, the tasks are written to the \textit{Executable Queue} 
% of the respective PE. 
% We note there is one \textit{Executable Queue} for each PE, 
% while the \textit{Ready Queue} and \textit{Outstanding Queue} are shared by all resources in DS3. 
% The task stays in the \textit{Executable Queue} until the data required for processing is received. 
% For example, processing of the head task starts after the PE receives the data from the main memory. 
% Similarly, the data may be read from a local cache if the predecessor task was executed in the same cluster.
% DS3 uses analytical models to estimate the memory access latency as a function of the source-destination addressed on the NoC and traffic load~\cite{kiasari2013analytical}. 
% The details are omitted since analytical models are out of scope of this paper and the DS3 kernel is not limited to any specific model.
% After the data dependencies are satisfied, the PE runs the task following the execution time profile given by the resource database. 
% If the PE supports multi-threading, it can run multiple tasks concurrently during this time.


% After the execution of a task finishes, it is written to the \textit{Retire Queue}. 
% Then, the simulation kernel clears the dependencies imposed by these tasks and removes them from the system. 
% If all the predecessors of a task waiting in the \textit{Outstanding Queue} retire, 
% then the kernel moves them to the \textit{Ready Queue}, as shown in Figure~\ref{queues}.
% This triggers a new scheduling decision and set of tasks which go through the steps mentioned in the previous paragraph. 

% The simulation kernel also calls the DTPM governor periodically at every decision epoch, 
% as summarized in the previous section. 
% The DTPM governor determines the power states of the PEs as a function of their current load and information provided by the resource database. 
% Subsequently, the kernel updates the power states of the PEs and resumes its operation, as shown in Figure~\ref{queues}.


==> files/introduction_backup.tex <==
\section{Introduction}

There are over two million smart phone and tablet apps as of the third quarter of 2018 \cite{Statista2018_apps}. Designers of mobile platforms must deliver both competitive performance and energy-efficiency while running these applications to remain in the market. 
Hence, mobile platforms are designed to provide peak performance for intensive applications (e.g., games) and high energy-efficiency for low-intensity workloads (e.g., email).


Modern heterogeneous mobile SoCs support multiple types of cores (e.g., Big/Little) 
and different voltage/frequency levels for each core. 
The full potential of these architectures can be realized only if 
these knobs are managed optimally at runtime as a function of active applications.
This is a challenging problem for two reasons.
First, the joint space of control actions grows exponentially with the number of cores and their frequency levels. For example, Snapdragon 810 SoC features four Little and four Big cores whose power states (on/off) and frequency levels can be controlled adaptively. 
Consequently, power management drivers need to choose one out of \jana{4128 feasible solutions} 
at every control interval, which typically ranges from 50 to 100~ms. 
Second, it is impractical to perform application-specific optimization due to the exponential growth of potential applications. 
Therefore, there is a great need for runtime techniques 
that can manage mobile SoCs optimally for a wide variety of applications.


%Modern heterogeneous mobile SoCs support multiple types of cores (e.g., Big/Little) and different voltage/frequency levels for each core. 
%Dynamic management allows us to appropriately trade-off performance and energy as per the needs of target applications. However, it is very challenging to automatically determine the optimum composition of active cores and their frequencies at runtime for the following two reasons. First, the joint space of control actions grows exponentially with the number of cores and their frequency levels. For example, Snapdragon 810 SoC features four Little and four Big cores whose power states (on/off) and frequency levels can be controlled adaptively. Consequently, power management drivers need to choose one out of \jana{4128 feasible solutions} at every control interval, which typically ranges from 50 to 100~ms. Second, it is impractical to perform application-specific optimization due to the exponential growth of potential applications. There is a great need for creating adaptive policies that will generalize well to new applications.

%A wide dynamic range in performance and energy-efficiency is enabled by heterogeneous architectures which support multiple core types (e.g., big/little) and voltage-frequency levels for each core. 
%However, the full potential of these architectures can be realized only if the optimum composition of the active cores and their frequencies are known at runtime. This is a challenging problem for two reasons. First, application-specific optimization is not feasible, as the space of potential applications, which is already huge, is expanding continuously. Similarly, the action space explodes since it grows with the cartesian product of the number of cores, their frequency levels and the types of cores. For example,  Snapdragon 810 SoC features four little and four cores whose power states (on/off) and frequency levels can be controlled independently. Consequently, power management drivers need to choose one out of 4000 feasible solutions at every control interval, which typically ranges from 50~ms to 100ms. 

Despite the impressive progress in hardware support, existing solutions used in commercial systems 
still rely on simple heuristics. 
For example, interactive and powersave governors
increase (decrease) the operating frequency by one level when the utilization exceeds (goes below) a static threshold. 
More advanced algorithms ~\cite{martinez2009dynamic,muthukaruppan2013hierarchical,muck2017hetero, donyanavard2016sparta} have failed to replace these simple solutions for two primary reasons. 
First, one of the main differentiating factors is still the performance perceived by the user, such as touch responsiveness or the maximum throughput while running key performance indicators (KIP). 
Hence, the interactive governor, the default policy employed by Android phones, is very aggressive in driving the frequency levels up. Since this choice leads to running at highest frequencies during most of the active time of applications, there is almost no room for improving the performance. Second, it is hard to beat the simplicity of the existing governors, even though energy-efficiency, measured in performance per watt (PPW), can be improved significantly. 
Therefore, new solutions must 
not only \textit{dominate} the existing governors in the performance versus energy-efficiency solution space, but also be \textit{practical}. 

%, still rely on simple heuristics based on core utilization. For instance, they increase (decrease) the operating frequency by one level when the utilization exceeds (goes below) a static threshold. Nevertheless, more advanced algorithms ~\cite{martinez2009dynamic,muthukaruppan2013hierarchical,muck2017hetero, donyanavard2016sparta} have failed to replace these simple solutions for two primary reasons. First, one of the main differentiating factors is still the performance perceived by the user, such as touch responsiveness or the maximum throughput while running key performance indicators (KIP). Hence, the interactive governor, the default policy used by Android phones, is very aggressive in driving the frequency levels up. Since this choice leads to running at the highest frequencies during most of the active time of the applications, there is almost no room for improving the performance. Second, it is hard to beat the simplicity of the existing governors, even though the energy-efficiency, measured in performance per watt, can be improved significantly. Therefore, the competing algorithms must be both \textit{practical} and \textit{superior to existing governors}, i.e., dominate them in the performance versus energy-efficiency plane. 

In this paper, we present a \textit{novel and practical} dynamic management technique for heterogeneous mobile platforms using 
the imitation learning (IL) framework~\jana{\cite{sutton and another one}. 
IL is a promising approach since 
it enables us to bridge an optimal offline solution with an efficient online policy. 
Reinforcement Learning (RL) based methods such as Q-learning with lookup tables have been considered by prior work as an alternative~\cite{chen2015distributed, ul2017hybrid}. However, prior RL based solutions have following drawbacks: 1) They are not practical as the size of the Q-table grows exponentially with the state and action space, as we demonstrate in our experimental results section. As a result, they require huge storage, which is limited on mobile platforms; 2) Performance of RL methods depend critically on the design of a good reward function to drive the learning process, which is a non-trivial task; 3) The overall learning process to create near-optimal policies is very slow due the need to try different actions at each state (i.e., exploration) to discover the best decision. 

IL is a significantly better framework than RL to create adaptive policies \cite{sun2017deeply}: requires less time and training data; allows us to leverage off-the-shelf classification/regression algorithms; and policies are stored in the form of parametric or non-parametric functions that have minimal storage requirements. However, IL requires the creation of an oracle policy meeting the designer's goals to provide the training data that is necessary to drive the learning process. Therefore, we provide an efficient mechanism to construct near-optimal oracle policies {\em offline} to optimize a given objective. First, we instrument a set of benchmark applications, which are known to the designers, such that we can collect performance counters for a block of macroblocks~\cite{lattner2004llvm}, referred as {\em snippets}. Second, we run the instrumented applications at different configurations supported by the platform and measure the corresponding power consumption. In this way, we obtain the power consumption and performance counters, including the number of instructions and active cycles, for each snippet. Third, we construct a near-optimal oracle policy using the rich set of collected data to minimize a specified objective such as PPW noting that other metrics (e.g., energy consumption) can be employed as needed. The oracle policy corresponds to the best configuration (control actions for all control knobs)  for each snippet to minimize PPW. We employ advanced IL algorithms using the oracle to create low-overhead control policies that generalize well to unseen applications. 


%In the offline design stage, we first instrument a set of benchmarks, which are known to the designers, such that we can collect performance counters for a block of macroblocks~\cite{lattner2004llvm}, called snippets. Then, we run the instrumented applications at different configurations supported by the platform while measuring the power consumption. In this way, we obtain the power consumption and performance counters, including the number of instructions and active cycles, for each snippet. The resulting rich set of data enables us to construct an oracle that reveals the optimum configuration for each snippet with respect to PPW\footnote{We note that one can choose any optimization metric, such as energy consumption,  that can be computed using the collected data}. The last step of the offline design stage is using imitation learning to design a low-overhead global policy with the help of the oracle. 


%Our solution is enabled by an extensive offline design stage and efficient implementation that runs online. In the offline design stage, we first instrument a set of benchmarks, which are known to the designers, such that we can collect performance counters for a block of macroblocks~\cite{lattner2004llvm}, called snippets. Then, we run the instrumented applications at different configurations supported by the platform while measuring the power consumption. In this way, we obtain the power consumption and performance counters, including the number of instructions and active cycles, for each snippet. The resulting rich set of data enables us to construct an oracle that reveals the optimum configuration for each snippet with respect to PPW\footnote{We note that one can choose any optimization metric, such as energy consumption,  that can be computed using the collected data}. The last step of the offline design stage is using imitation learning to design a low-overhead global policy with the help of the oracle. 

%Imitation learning is crucial in obtaining a practical policy that achieves near-optimal results. We note that reinforcement learning (RL) has been considered by prior studies as an alternative~\cite{chen2015distributed, ul2017hybrid}. For example, techniques based on Q-tables have convergence properties. However, they are not practical since the size of the Q-table, hence the storage requirements, explode with action space, as we demonstrate in our experimental results section. Moreover, RL techniques depend critically on designing a non-trivial reward function that guides the policy. Since the ground truth is not known at runtime, producing a reliable reward function is not practical. In contrast, our solution employs a decision tree that imitates the oracle. That is, it uses the correct labels provided by the oracle instead of relying on a reward function. We call the resulting as ``global'' since it learns from an ensemble of known applications. We also demonstrate that it performs well for the applications seen only at runtime. Our implementation on the Odroid XU3 platform demonstrates that it has less than \textcolor{red}{XX\%} implementation overhead. Furthermore, our evaluations with 16 commonly used benchmarks shows on average 80\% improvement in performance-per-watt (PPW). 

%\vspace{0.05in}

\noindent {\bf Contributions.} The main contributions of this paper include:
\begin{itemize}
    \item Construction of an Oracle policy using benchmark applications that are provided to aid the creation of control policy with desired behavior (e.g., minimizes PPW).

    \item Imitation learning (IL) based methodology using the constructed Oracle policy to automatically create practical power management governors that generalize to unseen applications.

    \item Empirical evaluation of the policies constructed using IL, their implementation overhead, and comparison to the state-of-the-art governors on a big.LITTLE hardware platform.
\end{itemize}




==> files/related_work.tex <==
% \section{Related Work} \label{sec:related work}

% % One of the most critical steps of system-level design of DSSoCs to achieve power-performance optimization is to address the resource and power-thermal management issues.
% %
% One of the most important goals of 
% heterogeneous SoC design % not just DSSoC
% is optimizing energy-efficiency while satisfying the performance constraints. % more specific goal.
% Indeed, a variety number of offline and runtime algorithms have been proposed to schedule applications to PEs in multicore architectures~\cite{KPN_map_MPSoCs, shao2005efficient, smit2005run, de2010dynamic,chou2008energy}. 
% Similarly, DVFS policies, such as HiCAP ~\cite{park2016hicap}, power management governors, such as Ondemand~\cite{pallipadi2006ondemand}, and thermal management techniques~\cite{coskun2008temperature} have been proposed to efficiently manage the power and temperature of SoCs.
% However, existing approaches are typically evaluated in isolated environments and different in-house tools.
% Hence, there is a strong need for a unified simulation framework~\cite{maurya2018benchmarking}
% % However, as others like Maurya and Tripathi note , there is a strong need 
% to compare and evaluate various scheduling and optimization algorithms in a common environment.
% % However, existing approaches are evaluated in isolated/different in-house tool.
% % Isolating the scheduler within a simulation framework allows architects to evaluate a wide range of scheduling algorithms at design time and identify the algorithm that is most suitable for the target domain and performance objectives.
% %However, there is a strong need for comparison of different approaches to scheduling at design time to choose the best algorithm for implementation suitable for the domain. 

% A number of full system simulators have been developed to simulate the entire SoC using functional models for the key components, 
% such as cores, interconnect, and memories. 
% For example, gem5 \cite{binkert2011gem5} is a widely used CPU architecture simulator with GPU extensions~\cite{power2015gem5-gpu}. While it provides architectural support for ARM and is suitable for SoC simulations, it lacks support for general heterogeneous architectures, even with the capabilities of gem5-gpu. 
% Moreover, its slow speed severely limits the scope of design space explorations and prohibits meaningful thermal analysis.
% Such full system simulators also involve a steep learning curve and significant developmental effort with little to no support for plug and play options, inhibiting its use for rapid exploration.
% Several SystemC-based simulation frameworks enable SoC exploration~\cite{spatial,beltrame2009resp}. For example, the framework presented in~\cite{spatial} allows representing applications as high-level state machines and conducting timing emulation of multi-threaded SoC platforms. Similarly, a lower-level instruction set based simulation approach is taken by \cite{beltrame2009resp}. 
% % Please check the following. Do you mean "these frameworks"? 
% % If this applies only to the second tool, why is the first one not sufficient for DSSoC?
% However, these frameworks are restricted to applications that are already implemented in SystemC.

% StarPU \cite{augonnet2011starpu} is a comprehensive framework that provides the ability to perform run-time scheduling and execution management for directed acyclic graph (DAG) based programs on heterogeneous architectures. It is, notably, integrated into SimGrid \cite{casanova2013simgrid} framework. 
% However, SimGrid was developed in the context of providing fast simulation for distributed systems, and the authors acknowledge that it is not intended to scale down to simulating real-time multi-threaded systems or comparing kernel schedulers and policies \cite{simgrid-limits}.
% % This looks like SimGrid limitation. What is wrong with StarPU (like spatial)?
% %
% %TODO Josh: Would this last simgrid-limits citation be better as a footnote?
% A recent work targets domain-specific programmability of heterogeneous architectures through intelligent compile-time and run-time mapping of tasks across CPUs, GPUs, and hardware accelerators. 
% To demonstrate the proposed approach, the authors employ three different simulators, more specifically, 
% Contech~\cite{railing2015contech} to generate traces, MacSim~\cite{kim2012macsim} to model CPU/GPU architectures, and BookSim2~\cite{booksim} to model the networks-on-chip. 
% The proposed DS3 framework would benefit this and other similar studies by providing a single integrated simulation framework. 

% % Another simulation framework for temporal and spatial task mapping on MPSoC platforms has been developed in \cite{spatial}.
% % ReSP \cite{beltrame2009resp} is a SystemC-based simulation framework for MPSoC platforms that utilizes instruction-set simulation to integrate existing SystemC components without any source-code modifications. 
% %A result of this, though, is that applications are required to have SystemC implementations to be mapped to this framework, which can add initial costs to design space exploration if no existing implementation is available.

% To the best of our knowledge, DS3 is the first integrated open-source framework to address rapid system-level power, performance, and temperature exploration of DSSoCs. 
% It includes not only built-in analytical models, scheduling algorithms, and DTPM policies, but also five reference applications from wireless communication and radar processing domain.
% % 
% % Dr. Marculescu: need to say it can directly work w/ complex FPGAs like Zynq board 
% %  

% % todo{Finish with what is unique about DS3. What should someone care to read this paper instead of other prior work?}


